MixMo: Mixing Multiple Inputs for Multiple Outputs via Deep Subnetworks

Recent strategies achieved ensembling "for free" by fitting concurrently diverse subnetworks inside a single base network. The main idea during training is that each subnetwork learns to classify only one of the multiple inputs simultaneously provided. However, the question of how to best mix these multiple inputs has not been studied so far. In this paper, we introduce MixMo, a new generalized framework for learning multi-input multi-output deep subnetworks. Our key motivation is to replace the suboptimal summing operation hidden in previous approaches by a more appropriate mixing mechanism. For that purpose, we draw inspiration from successful mixed sample data augmentations. We show that binary mixing in features - particularly with rectangular patches from CutMix - enhances results by making subnetworks stronger and more diverse. We improve state of the art for image classification on CIFAR-100 and Tiny ImageNet datasets. Our easy to implement models notably outperform data augmented deep ensembles, without the inference and memory overheads. As we operate in features and simply better leverage the expressiveness of large networks, we open a new line of research complementary to previous works.

==> pictures/experiments/feat_app.tex <==
% \begin{figure}
%   \includegraphics[width=\linewidth]{pictures/experiments/feat_plots/mixmo2810cx_mimor_layer1}
%   \caption{The projections heads clearly differentiate the two inputs in the
%     fusion space.}
% \end{figure}
\begin{figure}
\centering
\begin{subfigure}[b]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{pictures/experiments/files/mimo2810L1}
\caption{Filters $l_1$-norms of the input encoders $c_0$ and $c_1$.}
\label{fig:mixmo_proj}
\end{subfigure}
\hfill%
\begin{subfigure}[b]{0.48\columnwidth}%
\centering%
\includegraphics[width=\columnwidth]{pictures/experiments/files/mixmo2810cx_mimor_layer1.png}%
\caption{$Var(c|x_{0/1})$ with respect to inputs $x_0$ and $x_1$.}%
\label{fig:active_feats}%
\end{subfigure}%
\caption{\textbf{Repartition of inputs in the shared latent space}. Both a network based study (filter norms, see Sec.~\ref{sec:msdamixmo}) and an input based study (conditional variances) show the same separation in the shared latent space.}
\label{fig:active_app}
\end{figure}

==> pictures/experiments/fig_active_features.tex <==
\begin{figure}[!t]%
\centering%
\includegraphics[width=1.0\linewidth]{pictures/experiments/files/width_acc_active.jpg}%
\caption{\textbf{Parameters Efficiency}. CIFAR-100 with WRN-28-$w$. Proportion of active filters ($l_{1}$-norm $>0.4$ of max in layer \cite{li2017pruning}) decreases in larger vanilla networks. Yet, Cut-MixMo better leverages over-parametrization. If $w>2$ (resp.\ $w\geq4$), Cut-MixMo is better than a vanilla network (resp.\ deep ensembles, despite 2 times less parameters).}%
\label{fig:activefeaturesacc}%
\end{figure}%
% \caption{\textbf{Parameters Efficiency} on CIFAR-100 with WRN-28-$width$. Proportion of active filters \cite{li2017pruning} (L1 norm $\geq$ 40\% of max in layer) is reduced in larger networks. Cut-MixMo improves performance by reducing this phenomenon. If $w>2$ (resp.\ , Cut-MixMo is better than a vanilla network. If $w\geq4$, Cut-MixMo is better than deep-ensembles despite 2 times less parameters.}%

==> sections/sections_deprecated/03_model_reweight_mtl.tex <==
Asymmetries in the mixing mechanism can cause one
input to overshadow the other. Notably when $\kappa \ne 0.5$, the predominant input may be easier to predict.
We seek a weighting function $w_r$ to \textbf{balance the relative importance} of the two $\mathcal{L}_{\text{CE}}$ in
$\mathcal{L}_{\text{MixMo}}$. It modifies the effective learning rate, how gradient flows in the network and overall how mixed information is represented in features.
Interestingly, this is a central theme in \textbf{multi-task learning} \cite{caruana1997multitask}: while it aims at predicting several
tasks from a shared input, we predict a shared task from several different inputs.
Beyond this chiastic structure, we face similar issues. In particular, information separation from a shared representation is challenging.
Moreover, gradients for one task can be detrimental to another conflicting task \cite{kendall2018multi,sener2018multi,chen2018gradnorm}.
% \alex{Weights are usually not normalized by the number of tasks in MTL\cite{chen2018gradnorm,guo2018dynamic}.}
Fortunately, MixMo presents a distinct advantage: the exact ratios $\kappa$ and $1-\kappa$ of each task are known exactly.% 

We therefore leverage $\kappa$ to weight via:%
\begin{equation}%
w_{r}(\kappa) = 2\frac{\kappa^{1/r}}{\kappa^{1/r} + (1-\kappa)^{1/r}}.
\end{equation}%
This defines a family of functions by varying the parameter $r$, visualized for $r=3$ in red in Fig.~\ref{fig:archi_network} (more in Appendix \ref{app:weighting}). This power law provides a natural relaxation between \textbf{two extreme configurations}. The first extreme, $r=1$, $w_{1}(\kappa)=2\kappa$, is in line with linear label interpolation in MSDA. The resulting imbalance in each subnetwork's contribution to $\mathcal{L}_{\text{MixMo}}$ causes lopsided updates. While it promotes diversity, it also reduces regularization: the overshadowed input has a reduced impact on the loss. The opposite extreme, $r\to\infty$, $w_{\infty}(\kappa)\to1$, removes reweighting. Consequently, $w_r$ inflates the importance of hard minority inputs, à la Focal Loss \cite{lin2017focal}. However, minimizing the role of the predominant inputs destabilize training. Overall, we empirically observe that in-between $r$ perform best as they trade off pros and cons from both extremes.%
% - also used in multi-task learning \cite{mordan2020etecting} - 

==> tables/ablation_featdesc.tex <==
\begin{table}[!t]
  \caption{Description of distribution of variances over channels.}
\centering
\resizebox{0.9\linewidth}{!}{%
        \begin{tabular}{c c c c c c c}
            \toprule
          Layer & Approach & Width & Mean & Median & Min & Threshold \\ \midrule
          \multirow{12}{*}{$\mathcal{M}$} & \multirow{6}{*}{Vanilla} & 2 & 0.252 & 0.197 & 0.060 & 93.75 \\
                & &  3 & 0.205 & 0.137 & 0.071 & 87.50 \\
                & &  5 & 0.150 & 0.100 & 0.062 & 75.00 \\
                & &  7 & 0.135 & 0.121 & 0.046 & 75.00 \\
                & &  10 & 0.116 & 0.085 & 0.032 & 68.75 \\
                & &  14 & 0.093 & 0.065 & 0.014 & 43.75 \\ \cmidrule{2-7}
                & \multirow{6}{*}{Cut-MixMo} & 2 & 0.809 & 0.676 & 0.407 & 100.00 \\
                & &  3 & 0.701 & 0.607 & 0.420 & 100.00 \\
                & &  5 & 0.557 & 0.533 & 0.426 & 100.00 \\
                & &  7 & 0.459 & 0.399 & 0.287 & 100.00 \\
                & &  10 & 0.381 & 0.358 & 0.308 & 100.00 \\
                & &  14 & 0.324 & 0.311 & 0.235 & 100.00 \\ \midrule
          \multirow{12}{*}{Block 1} & \multirow{6}{*}{Vanilla} & 2 & 0.049 & 0.050 & 0.019 & 100.00 \\
                & &  3 & 0.025 & 0.024 & 0.005 & 97.92 \\
                & &  5 & 0.010 & 0.010 & 0.002 & 82.50 \\
                & &  7 & 0.006 & 0.005 & 0.000 & 70.54  \\
                & &  10 & 0.004 & 0.003 & 0.000 & 51.88 \\
                & &  14 & 0.002 & 0.002 & 0.000 & 43.75 \\ \cmidrule{2-7}
                & \multirow{6}{*}{Cut-MixMo} & 2 & 0.125 & 0.101 & 0.015 & 96.88 \\
                & &  3 & 0.076 & 0.078 & 0.015 & 91.67 \\
                & &  5 & 0.034 & 0.033 & 0.004 & 97.50 \\
                & &  7 & 0.018 & 0.017 & 0.003 & 94.64 \\
                & &  10 & 0.010 & 0.009 & 0.002 & 88.12 \\
                & &  14 & 0.005 & 0.004 & 0.001 & 76.79 \\ \bottomrule
          % \multirow{12}{*}{Layer 3} & \multirow{6}{*}{Cut-MixMo} & 2 & & &\\
          %       & &  3 & & & \\
          %       & &  5 & & & \\
          %       & &  7 & & & \\
          %       & &  10 & & & \\
          %       & &  14 & & & \\ \cmidrule{2-6}
          %       & \multirow{6}{*}{Linear-MixMo} & 2 & & & \\
          %       & &  3 & & & \\
          %       & &  5 & & & \\
          %       & &  7 & & & \\
          %       & &  10 & & & \\
          %       & &  14 & & & \\ \midrule
          % \multirow{12}{*}{Layer 4} & \multirow{6}{*}{Cut-MixMo} & 2 & & &\\
          %       & &  3 & & & \\
          %       & &  5 & & & \\
          %       & &  7 & & & \\
          %       & &  10 & & & \\
          %       & &  14 & & & \\ \cmidrule{2-6}
          %       & \multirow{6}{*}{Linear-MixMo} & 2 & & & \\
          %       & &  3 & & & \\
          %       & &  5 & & & \\
          %       & &  7 & & & \\
          %       & &  10 & & & \\
          %       & &  14 & & & \\
        \end{tabular}
    }
\label{table:featdesc}
\end{table}

==> tables/main_cifar10010_end_backup.tex <==
\begin{table}[!t]
\caption{\textbf{WRN-28-10 on CIFAR} without early stopping.}
\centering
\resizebox{0.8\linewidth}{!}{%
        \begin{tabular}{c | c | c c c | c c}
            \toprule
            \multicolumn{2}{c|}{Dataset} & \multicolumn{3}{c|}{CIFAR-100} & \multicolumn{2}{c}{CIFAR-10} \\
            \midrule
            \midrule
            Approach & \begin{tabular}{@{}c@{}}\scalebox{1.0}{Time}\\\scalebox{1.0}{Tr./Inf.}\end{tabular} & \begin{tabular}{@{}c@{}}\scalebox{1.0}{Top1}\\\scalebox{1.0}{$\%$}\end{tabular} & \begin{tabular}{@{}c@{}}\scalebox{1.0}{Top5}\\\scalebox{1.0}{$\%$}\end{tabular} & \begin{tabular}{@{}c@{}}\scalebox{1.0}{NLL$_{c}$}\\\scalebox{1.0}{$10^{-2}$}\end{tabular} & \begin{tabular}{@{}c@{}}\scalebox{1.0}{Top1}\\\scalebox{1.0}{$\%$}\end{tabular} & \begin{tabular}{@{}c@{}}\scalebox{1.0}{NLL$_{c}$}\\\scalebox{1.0}{$10^{-2}$}\end{tabular} \\
            \midrule
            \midrule
            Vanilla & \multirow{6}{*}{1/1} & 81.47 & 95.57 & 73.6 & 96.31 & 12.5 \\
            Mixup & & 83.15 & 95.75 & 66.3 & 97.00 & 11.3 \\
            Man.-Mixup$^\dagger$ & & 81.65 & - & - & 96.95 & - \\
            Hard PatchUp$^\dagger$ & & 83.87 & - & - & 97.47 & - \\
            CutMix & & 83.74 & 96.18 & 65.4 & 97.21 & 9.7 \\
            CowMix & & 83.00 & 95.95 & 67.3 & 97.24 & 9.7 \\
            \midrule
            Puzzle-Mix$^\dagger$ & 2/1 & 84.05 & 96.08 & 66.9 & - & - \\
            \midrule
            GradAug$^\dagger$ & \multirow{2}{*}{3/1} & 83.98 & 96.28 & - & - & - \\
            + CutMix$^\dagger$ & & 85.25 & 96.85 & - & - & - \\
            % \midrule
            % Vanilla BA$^\dagger$ & \multirow{2}{*}{8/1} & 83.45 & - & - & 97.15 &-  \\
            % Mixup BA$^\dagger$ & & 84.30 & - & - & \textbf{97.80} &- \\
            \midrule
            DE (2 Nets) & \multirow{2}{*}{2/2} & 83.15 & 96.30 & 66.0 & 96.58 & 11.1 \\
            + CutMix & & 85.46 & 96.90 & 57.4 & 97.51 & 8.7 \\
            \midrule
            \midrule
            \multirow{1}{*}{MIMO} & \multirow{5}{*}{2/1} & 82.04 & 95.75 & 69.1 & 96.33 & 12.1 \\
            \cmidrule{1-1}
            \cmidrule{3-7}
            \multirow{1}{*}{Linear-MixMo} & & 81.88 & 95.97 & 67.8 & 96.55 & 11.4 \\
            + CutMix & & 84.55 & 96.95 & 57.4 & 97.34 & 8.9 \\
            \cmidrule{1-1}
            \cmidrule{3-7}
            \multirow{1}{*}{Cut-MixMo} & & 84.07 & 96.97 & 56.6 & 97.26 & 8.7 \\
            + CutMix & & 85.17 & 97.28 & 54.4 & 97.33 & 8.5 \\
            \midrule
            \multirow{1}{*}{MIMO} & \multirow{5}{*}{4/1} & 82.74 & 95.90 & 67.0 & 96.66 & 11.5 \\
            \cmidrule{1-1}
            \cmidrule{3-7}
            \multirow{1}{*}{Linear-MixMo} & & 82.53 & 96.08 & 65.8 & 96.78 & 10.8 \\
            + CutMix & & 85.24 & 96.97 & 56.3 & 97.53 & 8.8 \\
            \cmidrule{1-1}
            \cmidrule{3-7}
            \multirow{1}{*}{Cut-MixMo} &  & 85.32 & 97.12 & 53.6 & 97.42 & 8.1 \\
            + CutMix & & 85.59 & 97.33 & 53.2 & 97.70 & 8.0 \\
            \bottomrule%
        \end{tabular}%
}%
\label{table:cifar10010end}%
\end{table}%

